Absence of percolation in graphs based on stationary point processes with degrees bounded by two

We consider undirected graphs that arise as deterministic functions of stationary point processes such that each point has degree bounded by two. For a large class of point processes and edge-drawing rules, we show that the arising graph has no infinite connected component, almost surely. In particular, this extends our previous result for SINR graphs based on stabilizing Cox point processes and verifies the conjecture of Balister and Bollob\'as that the bidirectional $k$-nearest neighbor graph of a two-dimensional homogeneous Poisson point process does not percolate for $k=2$.

==> Sec-Intro.tex <==
\section{Adaptive and decentralized transmission radii}
%The third case study is a continuation of the first two case studies to a more complicated connection model, where the transmission radii are not constant. 
We will now consider a model when the communication radius at a given user depends on the density of other users in the vicinity.  This assumption is not incorporated into models based on continuum percolation, and rarely other models. Continuum percolation was born out of a wireless network model by Gilbert~\cite{G61} who showed the existence of giant components. Under a signal-to-interference-plus-noise-ratio (SINR) model, Gilbert's result was recently generalized~\cite{dousse2006percolation} by demonstrating that giant components can exist on so-called SINR graphs. Percolation theory and related coverage processes are usually studied with models consisting of either fixed or i.i.d disk (ie transmission) radii. However, such models do not incorporate the effects of power control schemes, which manage the transmission radii. Typically, to reduce interference, the transmission radius is reduced in configurations with high user density.

We suggest developing a percolation model where the radii increase such that each one covers a certain fixed number of users. To be more precise, we propose to define the density (with respect to the $n$-dimensional product of some a priori radius distribution) of the transmission radii $\{\rho_i\}_{1\le i\le n}$ corresponding to the users $\{x_i\}_{1\le i\le n}$ to be given by 
$$\exp\big(-\beta\sum_{i<j} v(|x_i-x_j|,\rho_i,\rho_j)\big),$$
where $\beta>0$ is a parameter and $v:[0,\infty)^3\to[0,\infty) $ is a suitable pair potential function. For instance, defining $v(x,\rho,\rho')=\max\{\rho+\rho'-x,0\}$ introduces a penalty for configurations with a substantial amount of overlap in the transmission radii. See also~\cite{quermass} for related models.

Naturally, introducing such power control schemes, which render network models more realistic, adds further complexity. It is hoped that such a novel model will be both mathematically interesting as well as useful in shedding light on large wireless networks with relevant power control schemes. 

Independently to our proposal, a Gibbs sampler has been proposed for optimizing cellular networks in terms of SINR values by first using a standard  stochastic geometry model~\cite{chen2010self,chen2011joint,chen2012gibbsian}. These early results show a seemingly promising way to optimize networks in a de-centralized manner, which has much appeal, and we believe our research experience and knowledge of statistical physics, which originally inspired Gibbsian algorithms, can contribute to this line of research.


%radius of a given user $x_i$ as $\exp(-\beta\sum_{j\ne i} v(|x_i-x_j|))$, for a suitable pair potential function $v:
%$\min\{1,R_\ell\}$, where $R_\ell$ is the distance of the given user to the $\ell$-th closest user (with closeness being understood in terms of the ordinary Euclidean distance). 
%We would be interested in how the answers to the questions raised in Sections~\ref{wp1} and~\ref{wp2} change when using the more refined model. Of course, this will depend crucially on the precise form of the pair potential function. 
%This will depend crucially on the parameter $\ell$, since the simple model can be considered as a special case of the refined model with $\ell=\infty$.

Let us start doing some calculations. Using Campbell's theorem, we have in the simple case where the interaction radii are exponentially distributed with parameter $\beta\sum_{i\in I}v(|X_i-x|)$
\begin{align*}
\E[\#\{X_i\in X\colon o\in B_{r_i}(X_i)\}]&=\lambda\int\d x\P(|x|\le r(\bar X\cup \bar x))\\
&=\lambda\int\d x\E[\frac{\int_0^{|x|}\d\rho \exp(-\beta\sum_{i\in I}v(|X_i-x|,\rho)}{\int_0^{\infty}\d\rho \exp(-\beta\sum_{i\in I}v(|X_i-x|,\rho)}]\\
%&=\lambda\int\d x\exp(\lambda\int\d y(\e^{-\beta|x|v(|y-x|)}-1))\\
\end{align*}




==> pack_def.tex <==
\usepackage[notref,notcite]{showkeys} 
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{amsmath} 
\usepackage[mathscr]{eucal}
\usepackage{amssymb,bbm}
%\usepackage{changes} 
\usepackage{srcltx} 
\usepackage{dsfont}
\usepackage{hyperref}
\usepackage{color}
\usepackage{enumerate}
\usepackage{tikz}
\usepackage{boldline}
\usepackage{comment}
\usepackage{lscape}
\usepackage{graphicx}

%% List of macros follows. 
\numberwithin{equation}{section}
\newcommand{\Proof}{\skip\noindent{\itshape Proof: }} 
\newcommand{\ProofEnde}{\hfill {$\square$}

}%{$\square$} 
\newcommand{\ExampleEnde}{\hfill {$\diamond$}}
\newenvironment{proofsect}[1] 
{\vskip0.1cm\noindent{\bf #1.}\hskip0.5cm} 
 
\def\la{\lambda}
\def\lcp{\lambda^{\rm pe}_{\rm c}}
\def\lcc{\lambda^{\rm cl}_{\rm c}}
\def\lcd{\lambda^{\rm di}_{\rm c}}
 
\def\lcvp{\lambda_{\rm vp}}
\def\lcve{\lambda_{\rm v}}
\def\lcdp{\lambda_{\rm dp}}
\def\lcde{\lambda_{\rm d}}
\def\lcnp{\lambda_{\rm np}}
\def\lcne{\lambda_{\rm n}}

\def\emptyset{\varnothing} 
%%%%% Doppelstrichsymbole 
%%%%% Konvergenzsymbole 
\def\ti{\to\infty} 
\def\fH{{\mathfrak H}} 
\def\fK{{\mathfrak K}} 
%%%%%Griechische Buchstaben 
\def\a{\alpha} 
\def\b{\beta} 
\def\g{\gamma} 
\def\G{\Gamma} 
\def\d{{\rm d}} 
\def\e{\varepsilon} 
\def\l{l} 
%\def\m{\mu} 
\def\n{\Xi} 
\def\r{\varrho} 
%\def\s{\ifmmode \sigma \else $\sigma$\fi} 
\def\S{\Sigma} 
\def\t{\tau} 
\def\th{\theta} 
\def\ph{\varphi} 
\def\phn{\mathsf{\phi}} 
\def\Phn{\Phi} 
\def\O{\Omega} 
\def\tO{\tilde{\Omega}} 
\def\u{\upsilon} 
\def\z{\zeta} 
\def\p{\partial} 
%%%%%%%%Abk\"urzungen%%%%%%%%%%%% 
\def\L{\Lambda} 
\def\cP{{\mathcal P}} 
\def\cR{{\mathcal R}} 
\def\cS{{\mathcal S}} 
\def\cT{{\mathcal T}} 
\def\cW{{\mathcal W}} 
\def\cU{{\mathcal U}} 
\def\cX{{\mathcal X}} 
%%%%%%%%%%%%%Schlangenversionen%%%%%%%%% 
\def\tnu{\tilde{\Xi}} 
\def\tmu{\tilde{\mu}} 
\def\tP{\tilde{P}} 
\def\tQ{\tilde{Q}} 
\def\tcF{\tilde{{\cal F}}} 
\def\tG{\tilde{{\cal G}}} 
\def\c{\mathfrak c} 
\def\inv{^{-1}} 
\def\diag{\mbox{\rm diag}} 
%Bbb fonts 
\newfam\Bbbfam 
\font\tenBbb=msbm10 
\font\sevenBbb=msbm7 
\font\fiveBbb=msbm5 
\textfont\Bbbfam=\tenBbb 
\scriptfont\Bbbfam=\sevenBbb 
\scriptscriptfont\Bbbfam=\fiveBbb 
\def\Bbb{\fam\Bbbfam \tenBbb} 
\def\mmax{m_{\max}}
\def\NN{\mathrm{NN}}
\def\one{\mathds{1}}

%új folyam
\def\dmax{d_{\max}}
\def\SINR{\mathrm{SINR	}}
 
\newcommand{\m}     {\mathfrak{m}} 
\newcommand{\C}     {\mathcal{C}} 
\newcommand{\R}     {\mathbb{R}} 
\newcommand{\Z}     {\mathbb{Z}} 
\newcommand{\N}     {\mathbb{N}} 
\newcommand{\M}     {\mathbb{M}} 
\renewcommand{\P}   {\mathbb{P}} 
\newcommand{\D}     {\mathbb{D}} 
\newcommand{\E}     {\mathbb{E}} 
\newcommand{\Q}     {\mathbb{Q}} 
\newcommand{\Po}    {{\rm{Po}}}
 \newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\counting} {\mathfrak{c}} 
\newcommand{\smfrac}[2]{\textstyle{\frac {#1}{#2}}}
\newcommand{\ind}{\mathds}

\newcommand{\RR}     {\mathfrak{R}} 

\def\1{{\mathchoice {1\mskip-4mu\mathrm l}      % Blackboard bold 1 
{1\mskip-4mu\mathrm l} 
{1\mskip-4.5mu\mathrm l} {1\mskip-5mu\mathrm l}}} 
\newcommand{\ssup}[1] {{{\scriptscriptstyle{({#1}})}}} 
\def\comment#1{} 
\newtheoremstyle{thm}{2ex}{2ex}{\itshape\rmfamily}{} 
{\bfseries\rmfamily}{}{1.7ex}{} 
 
\newtheoremstyle{rem}{1.3ex}{1.3ex}{\rmfamily}{} 
{\itshape\rmfamily}{}{1.5ex}{} 
 
 \newcommand{\sss}{\scriptscriptstyle}
 
% THEOREM, EQN etc. commands 
 
\renewcommand{\theequation}{\thesection.\arabic{equation}} 
 
\newtheorem{theorem}{Theorem}[section] 
\newtheorem{lemma}[theorem]{Lemma} 
\newtheorem{prop}[theorem] {Proposition} 
\newtheorem{cor}[theorem]  {Corollary}
\newtheorem{claim}[theorem] {Claim}


\newtheorem{conj}[theorem] {Conjecture} 
\newtheorem{step}{STEP} 
 
\theoremstyle{definition}
\newtheorem{defn}[theorem] {Definition} 
\newtheorem{example}[theorem] {Example}
\newtheorem{bem}[theorem] {Remark}
\newtheorem{remark}[theorem]  {Remark} 

 \newcommand{\s}{\sigma}
 
 
%\renewcommand{\section}{\secdef\sct\sect} 
%\newcommand{\sct}[2][default]{\refstepcounter{section} 
%\vspace{0.8cm} 
%\setcounter{equation}{0} 
%\centerline{ %\large 
%\large\scshape \arabic{section}.\ #1} 
%\vspace{0.2cm}} 
%\newcommand{\sect}[1]{ 
%\vspace{0.8cm} 
%\centerline{\large\scshape #1} 
%\vspace{0.2cm}} 
% 
%\renewcommand{\subsection}{\secdef \subsct\sbsect} 
%\newcommand{\subsct}[2][default]{\refstepcounter{subsection} 
%\nopagebreak 
%\vspace{0.5\baselineskip} 
%{\flushleft\bf \arabic{section}.\arabic{subsection}~\bf #1  } 
%\nopagebreak} 
%\newcommand{\sbsect}[1]{\vspace{0.1cm}\noindent 
%{\bf #1}\vspace{0.1cm}} 
\newcommand{\heap}[2]{\genfrac{}{}{0pt}{}{#1}{#2}} 
% 
%\renewcommand{\subsubsection}{% 
%\secdef \subsubsect\sbsbsect} 
%\newcommand{\subsubsect}[2][default]{% 
%\refstepcounter{subsubsection} 
%\nopagebreak 
%\vspace{0.1\baselineskip} 
%\nopagebreak 

%{\flushleft 
%\sffamily\slshape 
%\arabic{section}.\arabic{subsection}.\arabic{subsubsection} 
%\ % 
%\sffamily #1\/.}\ } 
%\newcommand{\sbsbsect}[1]{\vspace{0.1cm}\noindent 
%{\bf #1}\ } 
 
% MATHEMATICAL SYMBOLS: 
 
\renewcommand{\d}{{\rm d}} 
\newcommand{\opn}{\operatorname} 
\newcommand{\eps}{\varepsilon} 
\newcommand{\Leb}{{\rm Leb}} 
\newcommand{\Lebmu}{{{\rm Leb}_\mu}}
\newcommand{\Sym}{\mathfrak{S}} 
\newcommand{\id}{{\rm{id}}} 
\newcommand{\esssup}{{\operatorname {esssup}}} 
\newcommand{\essinf}{{\operatorname {essinf}}}
\newcommand{\supp}{{\operatorname {supp}}} 
\newcommand{\sym}{{\operatorname {sym}}} 
\newcommand{\dist}{{\operatorname {dist}}} 
\newcommand{\diam}{{\operatorname {diam}}} 
\newcommand{\const}{{\operatorname {cst.}\,}} 
\newcommand{\Tr}{{\operatorname {Tr}\,}}   
\newcommand{\per}{{\operatorname {per}\,}} 
\newcommand{\zero}{{\operatorname {zero}\,}} 
% model-related things
\newcommand{\SIR}{\mathrm{SIR}}
\newcommand{\STINR}{\mathrm{STINR}}
\newcommand{\tensor}{\mathop{\otimes}}
\newcommand{\disjointcup}{\mathop{\huge{\amalg}}}
\newcommand{\directsum}{\mathop{\oplus}} 
\def\ellmin{\ell_{\min}}
\def\ellmax{\ell_{\max}}
\def\supp{\mathrm{supp}}
\def\kmax{k_{\max}}
\def\kopt{K_{\rm{opt}}}
% Caligraph fonts 
\newcommand{\Acal}  {{\mathcal A}}
\newcommand{\Bcal}  {{\mathcal B}}
\newcommand{\Ccal}   {{\mathcal C }} 
\newcommand{\Dcal}   {{\mathcal D }} 
\newcommand{\Ecal}   {{\mathcal E }} 
\newcommand{\Fcal}   {{\mathcal F }} 
\newcommand{\Gcal}   {{\mathcal G }} 
\newcommand{\Hcal}   {{\mathcal H }} 
\newcommand{\Ical}   {{\mathcal I }} 
\newcommand{\Jcal}   {{\mathcal J }} 
\newcommand{\Kcal}   {{\mathcal K }} 
\newcommand{\Lcal}   {{\mathcal L }} 
\newcommand{\Mcal}   {{\mathcal M }} 
\newcommand{\Ncal}   {{\mathcal N }} 
\newcommand{\Ocal}   {{\mathcal O }} 
\newcommand{\Pcal}   {{\mathcal P }} 
\newcommand{\Qcal}   {{\mathcal Q }} 
\newcommand{\Rcal}   {{\mathcal R }} 
\newcommand{\Scal}   {{\mathcal S }} 
\newcommand{\Tcal}   {{\mathcal T }} 
\newcommand{\Ucal}   {{\mathcal U }} 
\newcommand{\Vcal}   {{\mathcal V }} 
\newcommand{\Wcal}   {{\mathcal W }} 
\newcommand{\Xcal}   {{\mathcal X }} 
\newcommand{\Ycal}   {{\mathcal Y }} 
\newcommand{\Zcal}   {{\mathcal Z }} 
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\renewcommand{\e}   {{\operatorname e }}

\definecolor{Red}{rgb}{1,0,0}
\def\red{\color{Red}}
\newcommand{\todo}[1]{{\red{[\small #1]}}}

\DeclareMathOperator{\capa}{cap}
% END OF LIST OF MACROS 
 
\setlength{\textheight}{8.4in} 
\setlength{\textwidth}{6.6in} 
\setlength{\topmargin}{0in} 
\setlength{\headheight}{0.12in} 
\setlength{\headsep}{.40in} 
\setlength{\parindent}{1pc} 
\setlength{\oddsidemargin}{-0.1in} 
\setlength{\evensidemargin}{-0.1in} 
 
% Format : 
\marginparwidth 40pt 
\marginparsep 0pt 
\oddsidemargin-5mm 
\topmargin -30pt 
\headheight 12pt 
\headsep 15pt 
\footskip 15pt 
%\textheight 625pt 
%\textwidth 170mm 
\textheight 670pt 
\textwidth 170mm 
\columnsep 10pt 
\columnseprule 0pt 
% 
\renewcommand{\baselinestretch}{1.05} 

